Learning Hybrid Dynamics Models With Simulator-Informed Latent States

Dynamics model learning deals with the task of inferring unknown dynamics from measurement data and predicting the future behavior of the system. A typical approach to address this problem is to train recurrent models. However, predictions with these models are often not physically meaningful. Further, they suffer from deteriorated behavior over time due to accumulating errors. Often, simulators building on first principles are available being physically meaningful by design. However, modeling simplifications typically cause inaccuracies in these models. Consequently, hybrid modeling is an emerging trend that aims to combine the best of both worlds. In this paper, we propose a new approach to hybrid modeling, where we inform the latent states of a learned model via a black-box simulator. This allows to control the predictions via the simulator preventing them from accumulating errors. This is especially challenging since, in contrast to previous approaches, access to the simulator's latent states is not available. We tackle the task by leveraging observers, a well-known concept from control theory, inferring unknown latent states from observations and dynamics over time. In our learning-based setting, we jointly learn the dynamics and an observer that infers the latent states via the simulator. Thus, the simulator constantly corrects the latent states, compensating for modeling mismatch caused by learning. To maintain flexibility, we train an RNN-based residuum for the latent states that cannot be informed by the simulator.

==> models.tex <==
\subsection{Models} \label{section:mathematics}
In this section, we will add the necessary background on the models and data that we consider. 

\paragraph{Damped system: }
The data $x(t)$ are generated by adding a sine wave and a second sine oscillations that is exponentially damped over time. 
This yields the system
\begin{equation}
x(t)= \sin(0.1 t)+2\exp(-0.01 t)\sin(t).
\end{equation}
For the simulator, a simple sine wave with slight mismatch in the amplitude is chosen.
This yields
\begin{equation}
s(t)=0.7 \sin(0.1 t).
\end{equation}
The signals are obtained, by evaluating at $t=0, \dots 400$ with a discretization $\Delta t = 0.1$. Further the observation data are corrupted with white noise with variance $0.1$.  
\paragraph{Double torsion pendulum: }
For system ii), we consider the data from \citet{lisowski}.
We artificially add a transient component again $\Delta x$ via
\begin{equation}
\Delta x(t)=\exp(-0.5 t)\sin(50 t),
\end{equation}
evaluated at the interval $t = 0,1,2, \dots$. 
\paragraph{Van der Pol oscillator: }
For experiment iv), we consider a Van-der-Pol oscillator with additional control input. 
The differential equation for the Van-der-Pol oscillator with external force is given as
\begin{equation}
\begin{pmatrix}
\dot{x}(t) \\
\dot{y}(t) \\
\dot{u}(t) \\
\dot{v}(t)
\end{pmatrix}
=
\begin{pmatrix}
y \\
-x+a(1-x^2)y+bu \\
v \\
-\omega^2 u
\end{pmatrix},
\end{equation}
where $a,b$ and $\omega$ are system parameters. 
We choose $a=5, b=80, \omega=7.0$ and initial conditions 
\begin{equation}
\begin{pmatrix}
\dot{x}_0 \\
\dot{y}_0 \\
\dot{u}_0 \\
\dot{v}_0
\end{pmatrix}
=
\begin{pmatrix}
-2 \\
1 \\
0.31 \\
1
\end{pmatrix}.
\end{equation}
The system is evaluated at $t=5,\dots,100$ with step size $\Delta t=0.1$. 

